Inferring Strings from Position Heaps in Linear Time

Position heaps are index structures of text strings used for the string matching problem. They are rooted trees whose edges and nodes are labeled and numbered, respectively. This paper is concerned with variants of the inverse problem of position heap construction and gives linear-time algorithms for those problems. The basic problem is to restore a text string from a rooted tree with labeled edges and numbered nodes. In the variant problems, the input trees may miss edge labels or node numbers which we must restore as well.

==> figs/fig_macro.tex <==
\makeatletter
\def\tikz@collect@children@foreach[#1]foreach#2in{%
  \pgfutil@ifnextchar\bgroup{%
    \tikz@collect@children@foreachbr{#1}{#2}%
  }{%
    \tikz@collect@children@foreachnbr{#1}{#2}%
  }%
}

\def\tikz@collect@children@foreachbr#1#2#3{%
  \pgfutil@ifnextchar\bgroup{%
    \tikz@collect@children@foreachA{#1}{#2}{#3}%
  }{%
    \tikz@collect@children@foreachA{#1}{#2}{#3}{}%
  }%
}

\def\tikz@collect@children@foreachnbr#1#2#3{%
  \pgfutil@ifnextchar\bgroup{%
    \tikz@collect@children@foreachAnbr{#1}{#2}{#3}%
  }{%
    \tikz@collect@children@foreachAnbr{#1}{#2}{#3}{}%
  }%
}

\def\tikz@collect@children@foreachAnbr#1#2#3#4{%
  \expandafter\def\expandafter\tikz@children@list\expandafter{\tikz@children@list\tikz@childrennodesnbr[#1]{#2}{#3}{#4}}%
  \c@pgf@counta=\tikznumberofchildren%
  \foreach#2in#3{%
    \global\advance\c@pgf@counta by1\relax%
  }%
  \tikznumberofchildren=\c@pgf@counta%
  \tikz@collect@children%
}

\def\tikz@childrennodesnbr[#1]#2#3#4{%
  \c@pgf@counta=\tikznumberofcurrentchild\relax%
  \setbox\tikz@tempbox=\box\tikz@figbox%
  \foreach#2in#3{%
    \tikznumberofcurrentchild=\c@pgf@counta\relax%
    \setbox\tikz@figbox=\box\tikz@tempbox%
    \tikz@childnode[#1]{#4}%
    \global\c@pgf@counta=\tikznumberofcurrentchild\relax%
    \global\setbox\tikz@tempbox=\box\tikz@figbox%
  }%
  \tikznumberofcurrentchild=\c@pgf@counta\relax%
  \setbox\tikz@figbox=\box\tikz@tempbox%
}

% style
\tikzset{%
  tree node/.style={circle, draw, inner sep=1pt, minimum size=4.5mm, font=\small},%
  every child node/.style={tree node},%
  efp/.style={draw, -stealth},%
  edge from parent/.style={efp},%
  efpn/.style={font=\small\ttfamily, fill=white, inner sep=1pt},%
  level 1/.style={level distance=13mm, sibling distance=20mm},%
  level 2/.style={level distance=10mm, sibling distance=10mm},%
  suffix link/.style={draw, -stealth, densely dashed},%
}

\newcommand{\@MakeTree}[1]{%
  child foreach \x/\i/\children in #1 {%
    node {$\i$} \@MakeTree{\children} \if\x\@empty\relax\else edge from parent node [efpn] {\x}\fi%
  }%
}

\newcommand{\MakeTree}[2][0]{%
  \node [tree node] (root) at (0,0) {$#1$} \@MakeTree{#2};%
}

\makeatother
